On the Complexity of Branching-Time Logics

We classify the complexity of the satisfiability problem for extensions of CTL and UB. The extensions we consider are Boolean combinations of path formulas, fairness properties, past modalities, and forgettable past. Our main result shows that satisfiability for CTL with all these extensions is still in 2-EXPTIME, which strongly contrasts with the nonelementary complexity of CTL* with forgettable past. We give a complete classification of combinations of these extensions, yielding a dichotomy between extensions with 2-EXPTIME-complete and those with EXPTIME-complete complexity. In particular, we show that satisfiability for the extension of UB with forgettable past is complete for 2-EXPTIME, contradicting a claim for a stronger logic in the literature. The upper bounds are established with the help of a new kind of pebble automata.

==> expressivity.tex <==
\section{Expressivity}


\begin{theorem}[\cite{EmersonH85,EmersonH86}]
$$\ub\lex\ubplus\lex\ctl\eex\ctlplus\lex\ectl\lex\ectlplus\lex\ctlstar$$
\end{theorem}

\begin{theorem}[\cite{HaferT87}]
$\ctlstar\eex\pctlstar$
\end{theorem}

\begin{theorem}[\cite{LaroussinieS95}]
\begin{eqnarray*}
	&\ctl\not\leex\uby\not\leex\ectlplus\\
	&\ctl\not\leex\ubs\not\leex\ectlplus\\
	&\ctlpluspn\eex\ctlplusp\eex\ctlpn\eex\ctlp\eex\ctl\\
	&\ectl\lex\ectlp\lex\ectlpn\lex\ectlplus\eex\ectlplusp\eex\ectlpluspn\\
	&\ubyp\lex\ubypn\mex\ctl\\
	&\pectlplus\lex\pectlplusn\eex\pctlstarn\eex\pctlstar
\end{eqnarray*}
\end{theorem}

\begin{corollary}[Things easy to get from the proofs of the results above]
\begin{eqnarray}
	& \ub\lex\ubp\label{eqn:ub_ubp}\\
	& \ubs\not\leex\ectlplusypn\label{eqn:ubs_ectlplusypn}\\
	& \pctl\not\lex\ubplusypn\notag\\
	& \ubplusypn\lex\pctln\notag\\
	& \ubplus\not\leex\ubyp\label{eqn:ubplus_ubyp}\\
	& \ubp\lex\ubplusp\notag\\
	& \ubp\not\leex\ubplus\label{eqn:ubp_ubplus}\\
	& \ubplus\lex\ubplusp\notag\\
	& \ubplusp\lex\ctl\label{eqn:ubplusp_ctl}
\end{eqnarray}
\end{corollary}
\begin{proof}
\begin{itemize}
	\item[(\ref{eqn:ub_ubp})] $\myE(\myF p\land\myG q)$ is not expressible in \ubplus \cite{EmersonH85}, but can be expressed in \ubp by $\ef(\myH q\land p\land \eg q)$.
	\item[(\ref{eqn:ubs_ectlplusypn})] $\myE(s\lor a\myU b)\myU r$ cannot be expressed in $\ectlplus\eex\ectlpluspn$ \cite{LaroussinieS95}. This should be easy to extend to include \myY: the difference in the structures should not be at the end.
	\item[(\ref{eqn:ubplus_ubyp})] The \ubplus-formula $\ef(a\land\myE(\myF b\land\myG c))$ cannot be expressed in \ubyp (cf. \cite{EmersonH85,LaroussinieS95}).
	\item[(\ref{eqn:ubp_ubplus})] $\myE(p\myU q)$ cannot be expressed in \ubplus \cite{EmersonH85}, but can be expressed in \ubp by $\ef(\myH p\land\ex q)$.
	\item[(\ref{eqn:ubplusp_ctl})] $\ef(a\land\myE b\myU c\land\myE b'\myU c')$ cannot be expressed in \ubplusp (cf. \cite{LaroussinieS95}).
\end{itemize}
\qed
\end{proof}

\begin{theorem}[What we have]
\begin{eqnarray*}
	& \ubpn\eex\ctl\\
	& \pctl\eex\pctlplus\\
	& \pctln\eex\pctlplusn
\end{eqnarray*}
\end{theorem}



\begin{theorem}[What we need]
\begin{eqnarray}
	& \ectl\stackrel{?}{\lex}\pctlplusn & \text{(by MFCS-paper)}\\
	& \pctl\stackrel{?}{\meex}\pctln \label{eqn:pctl_pctln}\\
	& \pectl\stackrel{?}{\meex}\pectln \label{eqn:pectl_pectln}\\
	& \pctl\stackrel{?}{\meex}\ubplusypn\\
	& \pctl\stackrel{?}{\meex}\ubypn\\
%	& \ubs\stackrel{?}{\lex}\ubypn\\
	& \ubypn\stackrel{?}{\lex}\ubplusypn\\
	& \ubplusyp\stackrel{?}{\lex}\ubplusypn\\
	& \ubypn\stackrel{?}{\eex}\ubplusyp\\
	& \ubplus\stackrel{?}{\lex}\ubs\\
	& \ubplusp\stackrel{?}{\lex}\ubs
\end{eqnarray}
\end{theorem}
\begin{proof} Some ideas:
\begin{itemize}
	\item Try to show that $\varphi:=\ef(c\land\myA(s\lor a\myU b)\myU r)$ cannot be expressed in \pectlplus (start with \ctl, then $\pctl(\eex\pctlplus)$ and finally \pectlplus). As $\varphi$ can be expressed in \pctln, this solves (\ref{eqn:pctl_pctln}) and (\ref{eqn:pectl_pectln}).
\end{itemize}
\qed
\end{proof}
